Espaces de configuration g\'en\'eralis\'es. Espaces topologiques $i$-acycliques. Suites spectrales "basiques"

The generalized (ordered) configuration spaces associated to a topological space $X$ are the spaces $\Delta_{\leq\ell}X^{m}:=\{(x_1,\ldots,x_{m})\in X^{m}\mid\#\{x_1,\ldots,x_{m}\}\leq \ell\}$ and $\Delta_{\ell}X^{m}:=\Delta_{\leq\ell}X^{m}\setminus \Delta_{\leq\ell-1}$. They are equipped with the action of the symmetric group $S_m$ permuting coordinates. When $X$ has no interior cohomology (i.e. is $i$-acyclic) we are able to compute explicitly the character formula of $S_m$ acting on the cohomology of these spaces, and if $X$ is furthermore a connected and oriented pseudomanifold of dimension $\geq2$ we generalize Church's representation stability theorem to the case of the families $\{\Delta_{\leq m-a}X^m\}_m$ and $\{\Delta_{\ell-a}X^m\}_m$. We show that, for fixed $a,i\in\mathbb N$, the families of representations $\{ S_m: H ^{i}(\Delta_{?m-a}X^{m})\}_{m}$ are monotone and stationary for $m\geq4i+4a$, if $d_{X}=2$, and for $m\geq2i+4a$, if $d_{X}\geq3$. The corresponding families of characters and Betti numbers are (hence) polynomial and the families of integers $\{\mathop{\rm Betti}_{i}({\Delta_{?m-a}X^{m} / S_m})\}_{m}$ are constant within the same range of integers $m$. We further show that the family $\{\mathop{\rm Betti}_{i}({\Delta_{m}X^{m}/ S_m})\}_{m}$ is constant for $m\geq 2i$, if $d_{X}=2$, and for $m\geq i$, if $d_{X}\geq3$. In particular, complex algebraic varieties whether they are smooth on not verify these generalizations of Church's stability theorems.

==> theo-2016-11-25.tex <==
% !TEX root = configuration-fr.tex
%!TEX encoding = MacOSRoman
%!TEX spellcheck = fr 



\subsectionline{Stabilité de $\set\Bettibm^{i}(\BFm(\Mg))/_{m}$, cas $i$-acyclique.} 
La proposition \ref{prop-stabilite-chi-bg} qui suit étudie la formule de $\chibm(\Fm (\Mg))(\alpha,T)$ indépendamment de toute théorie de représentation ou topologie. La formule dépend alors seulement de la donnée de $m$ et $\dMg\in\NN$ et de la suite des nombres de Betti compacts $\cg=(\cg_0,\ldots,\cg_\dMg)\dans\ZZ^{\dMg+1}$, on notera 
$$\chi(\cg)_{m}:=\chibm(\Fm (\Mg))(\alpha,T)\,.$$

\smallskip\noindent{\slshape\bfseries\boldmath Polynomialité de la famille $\chideg{i}(\cg)$. }\'Evaluée en $\alpha\in\Sm$, la formule de $\chi(\cg)_{m}$ donne le polynôme de $\ZZ[T,1/T]$ noté 
$$\chi(\cg)_{m}(\alpha)=\sumnl_{i\in\ZZ}\chideg{i}(\cg)_{m}(\alpha)\,T^{i}\,,
$$
d'où les familles de fonctions centrales 
$\chideg{i}(\cg)=\set \chideg{i}(\cg)_{m}:\Sm\to\ZZ/_{m}\,.$

\smallskip
On dira d'une famille de fonctions centrales
$\fgg=\set f_{m}:\Sm\to\ZZ/_{m}$
qu'elle est \expression{(éventuellement) polynomiale} s'il existe un polynôme $Q_{\fgg}\in\ZZ[\XX_1,\XX_2,\ldots]$ tel que $f_{m}(\alpha)=Q_{\fgg}(\alpha)$ pour tout $m$ (assez grand) et tout $\alpha\in\Sm$. Un tel $Q_{\fgg}$ est unique (\footnote{En\label{unicité-poly} effet, si $Q(\XX_1,\ldots,\XX_\ell)\in\ZZ[\cl \XX]$ est non nul, il existe $a_i\in\NN$ tels que $Q(a_1,\ldots,a_\ell)\not=0$. Il est alors facile de fabriquer des permutations $\alpha_{m}\in\Sm$, pour tout $m\geq\sum_{i} a_i\,i$, telles que $a_i=\XX_{i}(\alpha_{m})$, auquel cas $Q(\alpha_m)=Q(a_1,\ldots,a_\ell)$ et $Q$ n'est pas  éventuellement nulle.}) et le \expression{degré polynôme de $\fgg$} est alors celui de $Q_{\fgg}$. Si $f_m=Q_{\fgg}$ pour tout $m\geq N$, on dira 
que \expression{$\fgg$ est polynomiale sur $\set m\geq N/$}.


\def\vartitle{Critère de polynomialité}\begin{var}Soit\label{critere-poly} $\fgg(\XX_{i_1},\ldots,\XX_{i_\ell})$
une expression telle que pour tout $m$, la fonction
$f_{m}(\alpha):=\fgg(\XX_{i_1}(\alpha),\ldots,\XX_{i_\ell}(\alpha))$
soit bien définie sur $\Sm$ à valeurs dans $\ZZ$. Alors, pour que
la famille de fonctions centrales $\fgg=\set f_{m}:\Sm\to\ZZ/$ soit polynomiale sur $\set m\geq N/$, il est nécessaire que $\fgg(n_1,\ldots,n_\ell)$ soit un polynôme en les entiers $n_j\geq0$ tels que $\sum_j n_j\cdot i_{j}\geq N$.
\end{var}
\demo
Pour $\ng:=(n_{1},\ldots,n_{\ell})$, notons $|\ng|=\sum_j n_{j}\cdot i_{j}$ et choisissons $\sigma(\ng)\in\S_{|\ng|}$ vérifiant $\XX_{i_j}(\sigma(\ng))=n_j$, pour $1\leq j\leq \ell$. Alors, si $Q\in\ZZ[\XX_1,\XX_2,\ldots]$ est un polynôme tel que $f_m=Q$ sur tous les $\Sm$ tels que $m\geq N$, on a 
$$\fgg(n_1,\ldots,n_{\ell})=
f_{|\ng|}(\sigma(\ng))=Q(\sigma(\ng))=Q'(n_1,\ldots,n_{\ell})$$
où $Q'\in\ZZ[\YY_1,\ldots,\YY_\ell]$ est obtenu de $Q$ en posant $\YY_j:=\XX_{i_j}$ et en annulant les autres variables.
\enddemo


\smallskip
\noindent{\slshape\bfseries Factorielle décroissante modifiée. }On utilisera une extension de la notion de factorielle décroissante (\ref{factorielles}). 
Pour $a,b$ dans un anneau et $\XX\in\NN$, on note\glossary{${a\uspp{0}[b]=1\,,\quad\text{et}\quad
a\uspp \XX [b]:=a(a-h)(a-2h)\cdots(a-(\XX{-}1)h)}$:factorielle décroissante étendue}
$$a\uspp{0}[b]=1\,,\quad\text{et}\quad
a\uspp \XX [b]:=a(a-b)(a-2b)\cdots(a-(\XX{-}1)b)\,,
$$
On a alors: 
$
b^{\XX}a\uspp \XX[c]=(ba)\uspp \XX [bc]
$ et $
a\uspp {\XX+1} [b]=a\uspp {\XX} [b](a-\XX\, b)
\,.$




\comment
\medskip
D'autre part
$$%\preskip0pt
\Betti_{i}(\BFm(\Mg))={(-1)^{i}\over m!}\sum_{\alpha\in\Sm}{1\over i!}{\partial^{i}\over\partial T^{i}}\Big(\chibm(\Fm (\Mg))(\alpha,T)\Big)\vrule height15pt depth12pt{\vrule depth10pt width0pt}_{\,T=0}$$
Des formules qui, modulo le théorème de stabilité de caractères polynomiaux \ref{prop-rang-stabilite-caracteres}, réduisent la détermination du rang de stabilité de la famille $\set\Betti_{i}(\BFm(\Mg))/_{m}$, à celle du degré $\ddeg$ du terme en $T^{i}$ de la série
$$Q(\cl\XX,T):=\prod_{d=1}^{m}
\goodsmash{0.8}{0.5}{\Big({-}d
(-T)^{d(d_\Mg-1)}\Big){\vrule height 9pt width0pt}^{\XX_d} 
\Big({-}{1\over d}\sum_{e\div d}\mobius de
{\Pc(\Mg)(-T^{-e})\over -T^{-e}}\Big)\usp {\XX_d}}
\,.$$
\endcomment


%%%%%%%%%%%%
\begin{prop}
\'Etant\label{prop-stabilite-chi-bg} donnés $\dMg\in\NN$ et 
$\cg=\set\cg_{0},\ldots,\cg_{\dMg}/\dans\ZZ$, on note
$P_{\cg}(T)=\cg_0+\cg_1T+\cdots+\cg_{\dMg}T^{\dMg}$ et 
$$\chi(\cg)_{m}(\cl\XX,T):=
\prod_{d=1}^{m}\Big({(-T^{d})^{\dMg}\over d^{-1}\,T^{d}}\Big){\vrule height 12pt width0pt}^{\XX_d} 
\Big(\sum_{e\div d}\mobius de
{P_{\cg}(-T^{-e})\over d\,T^{-e}}\Big){\vrule height 12pt width0pt}\usp {\XX_d}\,.$$
Alors, pour tout $i\in\NN$, la famille $\chideg{i}(\cg)$ est éventuellement polynomiale
 si et seulement si, $\cg_{\dMg}\in\set0,1/$. Dans ce cas, on a les propriétés suivantes de $\chi(\cg)$ suivant les valeurs de $\dMg$.
$${\def\minipage#1{\vtop{\hsize8cm\parindent0pt#1}}
\def\tt#1 #2 {\vrule height#1pt depth#2pt width0pt}
\def\ligne#1 #2 #3{\tt#1 #2 \tt 10 4 $\bullet$ #3}
\def\hline{\noalign{\hrule}}
\vbox{
\halign{\vrule\tt15 6 \quad\hfil$#$\hfil\quad\vrule&\quad\minipage{#}\hfil\quad\vrule\crcr
\noalign{\hrule}
%%%
\tt0 8 \dMg&$\hfil\chideg i(\cg_0,\ldots,\cg_{\dMg})$
%%%%%%%
\cr\hline
%%%
0&
\ligne0 0 {$\ddeg\chideg {-i}(\cg_0{=}1)\leq2i\,,$\hfill$\forall i\geq0$}\\
\ligne0 8 {$\chideg {-i}(\cg_0{=}0)_{m}=0\,,$\hfill$\forall m\,,\forall i\geq0$}
%%%%%%%
\cr\hline
%%%
1&
\ligne15 0 {$\chideg {0}(\cg_0{=}0,\cg_1)=(\cg_1)\,\uspp{\XX_1}[-1]\prod_{d>1}0\,\uspp{\XX_d}[-d]$\,,}\\
\ligne0 8 {$\chideg {i}(\cg_0{=}0,\cg_1)_{m}=0\,,$\hfill$\forall m\,,\forall i>0$}
%%%%%%%
\cr\hline
%%%
2&
\ligne0 0 {$\ddeg\chideg {i}(\cg_0,\cg_1,\cg_2{=}1)\leq2i\,,$\hfill$\forall i\geq0$}\\
\ligne0 8 {$\chideg {i}(\cg_0,\cg_1,\cg_2{=}0)_{m}=0\,,$\hfill$\forall m>i\geq0$}
%%%%%%%
\cr\hline
%%%
\geq3&
\ligne0 0 {$\ddeg\chideg {i}(\cg_0,\ldots,\cg_{\dMg}{=}1)\leq i\,,$\hfill$\forall i\geq0$}\\
\ligne0 11 {$\ddeg\chideg {i}(\cg_0,\ldots,\cg_{\dMg}{=}0)\leq {i\over \dMg{-}1}\,,$\hfill$\forall i\geq0$}
%%%
\cr
\hline}}}$$
\end{prop}
%%%%%%%%%%%%%%%%%
\demo \let\displayboxit\relax
Pour $d\geq 1$, notons
$$
\leftbrace{-0.5mm}{8.mm}\mathalign{
\displaystyle\Q_{d}(\cg)(\XX_d,T)&:=&
%%%%
\Big({(-T^{d})^{\dMg}\over d^{-1}\,T^{d}}\Big){\vrule height 12pt width0pt}^{\XX_d} 
%%%%
&
\Big(\sumnl_{e\div d}\mobius de\,
{P_{\cg}(-T^{-e})\over d\,T^{-e}}\Big)
{\vrule height 12pt width0pt}\usp {\XX_d}\,,\\
%%%%
\noalign{\kern2pt}
%%%%%%%
\displaystyle
\hfill\R(\cg)_{d}(T)&:=&\Big({(-T^{d})^{\dMg}\over d^{-1}\,T^{d}}\Big) 
\hfill&
\Big(\sumnl_{e\div d}\mobius de\,
{P_{\cg}(-T^{-e})\over d\,T^{-e}}\Big)\,,\hfill
}
%\postskip0.5ex
\eqnnb\label{Eq-Rd}
$$
%%%%%
de sorte que 
(\footnote{On omet d'indiquer `$\cg$' lorsqu'il est sous-entendu superflu.})
$$%\preskip1ex
\Q_d=(\R_{d})\uspp{\XX_d}[
(-1)^{d_\Mg}dT^{d(d_\Mg{-}1)}]\,.
\eqnnb\label{Eq-Rd-rec}
%\eqno(\ast)
$$
Lorsque l'on évalue $\Q_{d}$ en $\alpha\in\Sm$, on a
$\XX_d(\alpha)\in\NN$ et le développent de la factorielle décroissante  génère une série 
$$\Q_{d}(\XX_d(\alpha),T)=\sumnl_{i\in\ZZ}\Qdeg{i}_{d}(\XX_d(\alpha))\,T^{i}$$
où \smash{$\Qdeg{i}_{d}$} définit la famille fonctions centrales 
\smashtop{$\set\Sm\ni\alpha\mapsto\Qdeg{i}_{d}(\XX_d(\alpha))\in\ZZ/_m$.}

\smallskip
Le terme $\R_{d}(\cg)$ dans \ref{Eq-Rd} vaut, suivant les cas $d=1$ ou $d>1$,
$$
\hskip-3.9mm
\leftbrace{2.5mm}{8mm}
\mathalign
{
%%%%%%%
%\binspace1
\hfill\R_{1}(\cg)(T)&=&
\hskip-3mm\sum_{0\leq j\leq \dMg}
\cg_{j}
\,(-T)^{(\dMg{-}j)}\,,\hfill\\
%%%
\hfill\R_{d}(\cg)(T)&=&
\hskip-3mm
\sum_{%\let\stacklhss\relax
\scriptstack{%e\div d\\
\vrule height7pt width0pt
0\leq j\leq \dMg\mrlap{\scriptstyle,\ j\not=1\,,\ e\div d}}}
%\hskip-2mm
\mobius de\ 
\cg_{j}(-1)^{d_\Mg-j}
\,T^{d(\dMg-1)-e(j-1)}\,.\hskip-7mm
}
\raiseeqnnb{15pt}\label{Eq-Rd-dev}
$$
Il s'agit de polynômes, en $T^{\pm}$, en $T$ si $\dMg>0$ et en $1/T$ si $\dMg=0$. Le coefficient du terme constant est $\cg_{\dMg}$, sauf si $\dMg=1$ et $d>1$ auquel cas il est nul. Ensuite, le premier terme non constant, de la forme $? T^{\epsilon\not=0}$, 
varie suivant les situations. Le calcul explicite à partir des formules \ref{Eq-Rd-dev} donne
\begin{itemize}
%%%
\item \noindent\rlap{Si $d=1$,}\hfill $(\forall\dMg)
\quad\hskip-2pt ? T^{\epsilon}=-\cg_{\dMg-1}\,T^{\pm}\,.$
\hfill\null
%%%
\item \leavevmode\rlap{Si $d>1$,}\hfill
$\preskip-1.5ex
\def\ss#1{\hbox to1em{\mathsurround0pt\hss$#1$}}
\let\strut\relax\left\{\ \mathalign{
%%%%%%%%%%%%%%%%
\dMg=0,\ &?T^{\epsilon}&=&
%%%
\ss{}\cg_0\, T^{-d(p-1)/p}\hfill\\
%%%%%%%%%%%%%%%%
\dMg=1,\hfill&?T^{\epsilon}&=&
%%%
\ss{-}\cg_0\,\mu(d)\, T\hfill\\
%%%%%%%%%%%%%%%%
\dMg=2,\hfill&?T^{\epsilon}&=&
%%%
\ss{}\cg_2\, T^{d(p-1)/p}\hfill\\
%%%%%%%%%%%%%%%%
\dMg\geq 3,\hfill&?T^{\epsilon}&=&
%%%
\ss{-}\cg_{\dMg-1}\, T^{d}\hfill\\
}\right.
%\eqnnb\label{Eq-Qds}
$\hskip3mm\hfill\null

\end{itemize}
d'où les expressions
$$\def\ss#1{\hbox to2cm{#1,\hss}}
\let\strut\relax\left\{\ \mathalign{
%%%%%%%%%%%%%%%%
\forall\dMg\ &\Q_{1}(\cg)&=&
%%%
\halfsmashtop{\big(?T^{\pm}+\cg_{\dMg}\big)\uspp{\XX_1}[(-1)^{\dMg}T^{(d_{\Mg}{-}1)}]}\hfill\\
%%%%%%%%%%%%%%%%
\dMg=0,\ &\Q_{d}(\cg)&=&
%%%
\relax{\big(?T^{-d(p-1)/p}+\cg_0\big)\uspp{\XX_d}[d\,T^{-d}]}\hfill\\
%%%%%%%%%%%%%%%%
\dMg=1,\hfill&\Q_{d}(\cg)&=&
%%%
\big(?T\big)\uspp{\XX_d}[-d]\hfill\\
%%%%%%%%%%%%%%%%
\dMg=2,\hfill&\Q_{d}(\cg)&=&
%%%
\big(?T^{d(p-1)/p}+\cg_{2}\big)\uspp{\XX_d}[d\,T^{d}]\hfill\\
%%%%%%%%%%%%%%%%
\dMg\geq 3,\hfill&\Q_{d}(\cg)&=&
%%%
\big(?T^{d}+\cg_{\dMg}\big)\uspp{\XX_d}[(-1)^{\dMg}d\,T^{d(\dMg{-}1)}]\hfill\\
}\right.\postdisplaypenalty10000
\eqnnb\label{Eq-Qds}$$
où $p$ désigne le plus petit facteur premier de $d$.

\smallskip
\noindent{\slshape$\bullet$ Conditions nécessaires à la polynomialité. }En dehors du cas $\dMg=1$ qui pose de problèmes particuliers, dans tous les autres cas, le critère de polynomialité \ref{critere-poly} appliqué aux expressions \ref{Eq-Qds} donne aussitôt la condition
$$\Big(\Qdeg i_{d}(\cg)\vcenter{\hsize3cm\footnotesize\advance\baselineskip-1pt\centering est éventuellement polynomiale\par}\Big)\Longrightarrow \Big(\cg_{\dMg}\in\set0,1/\Big)$$
En effet, c'est déjà clairement la condition pour que
$\Qdeg 0_{d}(\cg)=\cg_{\dMg}^{\XX_d}$ soit polynomial. Ensuite, 
par exemple dans les cas $\dMg\geq3$, le terme qui suit est
$\Qdeg d_{d}=?\cg_{\dMg}^{\XX_d{-}1}T^{d}$ où la même condition apparaît, etc\dots

\smallskip
\noindent{\slshape$\bullet$ Les cas $d_\Mg=1$. }On a $\cg=(\cg_0,\cg_1)$ et
$$\leftbrace{0.mm}{6mm}\mathalign{
\Q_1(\XX_1,T)&=&\big({-\cg_0}\,T+\cg_1\big)\uspp{\XX_1}[-1]\hfill\\\noalign{\kern-2pt}
\Q_d(\XX_d,T)&=&\Big({-\cg_0}\sumnl_{e\div d}\mobius de\, T^{e}\Big){\vrule height10pt width0pt}\uspp{\XX_d}[-d]\,,\text{ si $d>1$,}
}
$$
Le critère de polynomialité appliqué à $\Q_1$ nous emmène à regarder les produits de $n$ facteurs
$$\big({-\cg_0}\,T+\cg_1\big)\big({-\cg_0}\,T+\cg_1+1\big)\cdots\big({-\cg_0}\,T+\cg_1+(n-1)\big)\,.$$
Pour chaque $i>0$, le coefficient en $T^{i}$ du produit
est
$(-\cg_0)^{i}\big(\sum x_1\cdots x_{n-i}\big)$, où la somme concerne les $(n{-}i)$-uplets d'éléments deux à deux distincts de l'ensemble $\binspace0
\set \cg_1,\cg_1+1,\ldots,\cg_1+(n-1)/$. Une telle somme est donnée par un polynôme en $n$ de degré $\binspace0n-i+1$, le coefficient en question n'est pas polynomial, sauf évidemment si $\cg_0=0$ auquel cas on a
$$\leftbrace{-0.5mm}{6mm}\mathalign{
\Qdeg{0}_{1}(0,\cg_1)&=&\cg_1\uspp{\XX_1}[-1]
\hfill\\
\Qdeg{0}_{d}(0,\cg_1)&=&0\uspp{\XX_d}[-d]\hfill\\
}
\text{\quad et\quad }\Qdeg{i}_{d}(0,\cg_1)=0\,,\ \forall i\geq 1\,,\forall d\geq 1\,.
$$
Par conséquent, 
$$\leftbrace{-0.5mm}{6mm}\mathalign{\chideg{0}(0,\cg_1)&=&\cg_1\uspp{\XX_1}[-1]
\Big(\prodnl_{d>1}0\,\uspp{\XX_d}[-1]\Big)\\
\chideg{i}(0,\cg_1)&=&0\,,\quad \forall i>0\,.\hfill}$$

%\newpage

\smallskip
\noindent{\slshape$\bullet$ Les cas $d_\Mg\in\set0,2/$. }Pour $\cg$ respectivement $(\cg_0)$ et $(\cg_0,\cg_1,\cg_2)$ on a
$$\mathalign{
\hfill\Q_{d}(\cg_0)&=&\Big(\sumnl_{e\div d}\mobius de {\cg_0\over T^{d-e}}\Big)\uspp{\XX_d}[d/T^{d}]\,,\hfill\\\noalign{\kern-2pt}
\Q_{d}(\cg_0,\cg_1,\cg_2)&=&\Big(\sumnl_{e\div d}\mobius de 
\big({\cg_0\, T^{d+e}}+\cg_1\,T^{d}+{\cg_2\,T^{d-e}}\big)
\Big)\uspp{\XX_d}[d\,T^{d}]\,,
}$$
où l'on constate aussitôt l'égalité
$$\Q_{d}(\cg_0)(\XX_d,1/T)=\Q_{d}(0,0,\cg_0)(\XX_d,T)\,,\eqnnb\label{Eq-dMg-0<=>2}$$
qui réduit le cas $\dMg=0$ à un cas particulier de $\dMg=2$.

Pour $\dMg=2$, on a vu dans \ref{Eq-Qds} que l'on a les expressions
$$\leftbrace{-0.5mm}{6mm}\mathalign{
\Q_{1}(\cg)&=&\big(?\,T+\cg_2\big)\uspp{\XX_1}[T]\hfill\\\noalign{\kern-2pt}
\Q_d(\cg)&=&\big(?\,T^{d((p-1)/p)}+\cg_2\big)\uspp{\XX_d}[dT^{d}]\,,\text{ si $d>1$.}
}
\eqnnb\label{Qd-dM=2-b2=1}
$$
où seuls les cas $\cg_{2}\in\set0,1/$ nous intéressent.


\begin{itemize}
\item Pour $\cg_2=1$, on a  $\Qdeg{0}_{d}=1$. Ensuite, les propriétés élémentaires des factorielles décroissantes dans les expressions \ref{Qd-dM=2-b2=1} justifient les relations 
$$%\hss
%\binspace0
%\relspace0
\let\quad\relax
\mathalign{
\Q_1(\XX_1,T)-\Q_1(\XX_1{-}1,T)&=&
%\\&&\hskip-1.5cm{}
\Q_1(\XX_1{-}1,T)\,(?-(\XX_1{-}1))\, T\hfill\\
\Q_{d}(\XX_d,T)-\Q_{d}(\XX_d{-}1,T)&=&
%\\&&\hskip-1.5cm{}
\Q_{d}(\XX_d{-}1,T)\,(?\,T^{d((p-1)/p)}-?(\XX_d{-}1)\,T^{d})\,,}
$$
dont on déduit, pour tout $i\geq 1$,
$$\def\sss#1 {\hbox to1.5em{\hfill(#1)}}
\mathalign{
\sss i \ddeg\Qdeg{i}_{1}&\leq&2&+&\ddeg\Qdeg{i{-}1}_{1}\hfill\\
\sss ii \ddeg\Qdeg{i}_{d}&\leq&d&+&\sup\Bigset
\ddeg\Qdeg{i-d((p-1)/p)}_{d},\ 
d+\ddeg\Qdeg{i-d}_{d}/\,.}
$$
On peut alors prouver par induction sur $i$ que l'on a
$$%\preskip0ex
\mathalign{
\ddeg\Qdeg{i}_{d}(\cg_0,\cg_1,\cg_2{=}1)&\leq& 2i\,,&\quad\forall i\geq0\,,\forall d\geq1\,.
}\eqnnb\label{Eq-dMg=2-b2=1}
$$
En effet, pour $i=0$ l'assertion est claire puisque $\Qdeg 0_{d}=1$. Ensuite, si l'on suppose $\ddeg\Qdeg{i{-}1}_{1}\leq2(i{-}1)$, l'égalité (i) donne
$\ddeg\Qdeg i_{1}\leq 2i$. Pour $\Qdeg i_{d}$, on remarque que 
$2i-2d(p-1)/p\leq 2i-d\,,
$ puisque $1/2\leq(p-1)/p$, et, à l'aide de (ii), on tire
$$\ddeg\Qdeg i_{d}\leq d+\sup\bigset 2i-d,\ d +2(i-d)/=2i\,,$$
ce qui prouve \ref{Eq-dMg=2-b2=1}. Par conséquent,
$$
\displayboxit{
\mathalign{\ddeg\chideg{i}(\cg_0,\cg_1,\cg_2{=}1)&\leq& 2i\,,\quad\forall i\geq0\,,
}}$$
puisque
$\chideg{i}(\cg)=\sum_{i_1+i_2+\cdots=i}\Qdeg{i_1}(\cg)_{1}\,\Qdeg{i_2}(\cg)_{2}\cdots$. 
On en déduit
$$
\displayboxit{
\mathalign{
\ddeg\chideg{-i}(\cg_0{=}1)&\leq& 2i\,,\quad\forall i\geq0\,,}}$$
grâce à l'égalité \ref{Eq-dMg-0<=>2}.

%%%
\item Lorsque $\cg_2=0$, on a
$$\binspace0
\leftbrace{-0.5mm}{13mm}\mathalign{
\Q_1(\XX_1,T)&=&\big(\cg_{0}\,T^{2}+\cg_1\,T\big)\uspp{\XX_1}[T]=
(-T)^{\XX_1}(-\cg_0\,T-\cg_1)\uspp{\XX_1}[-1]\hfill\\\noalign{\kern4pt}
\Q_d(\XX_d,T)&=&\Big((-T^{d})\sumnl_{e\div d}\mobius de (-\cg_0)\,T^{e}\Big)\uspp{\XX_d}[dT^{d}]\,,\text{ si $d>1$,}\hfill\\
&=&\big(-T^{d}\big)^{\XX_{d}}
\Big(\sumnl_{e\div d}\mobius de (-\cg_0)\,T^{e}\Big)\uspp{\XX_d}[-d]
\hfill}
$$
ce qui montre que pour tout $m$, la fonction centrale
$$\chi(\cg_0,\cg_1,\cg_2{=}0):\Sm\to\ZZ[T]\postskip0pt$$
 coïncide avec
$$(-T)^{m}\chi(\cg_0,-\cg_1)
:\Sm\to\ZZ[T]\,.$$
En particulier, 
$$\displayboxit{\chideg{i}(\cg_0,\cg_1,\cg_2{=}0)_{m}=0\,,\quad\forall m> i\geq0\,,}$$
alors que $\chi(\cg_0{=}0)=\prod_{d\geq1}0\uspp{\XX_d}[d/T^{d}]$ et donc
$$\displayboxit{\chideg {-i}(\cg_0{=}0)_{m}=0
\,,\quad\forall m\geq1\,,\forall i\geq0\,.}$$
\end{itemize}

\smallskip
\noindent{\slshape$\bullet$ Les cas $d_\Mg\geq3$. }On suit la même démarche que pour le cas $\dMg=2$ en se restreignant (donc) aux cas où $\cg_{\dMg}\in\set0,1/$.
%%%
\begin{itemize}
\item Pour $\cg_{\dMg}=1$ et tout $d\geq1$, on a $\Qdeg{0}_{d}=1$, et grâce à \ref{Qd-dM=2-b2=1}, la relation
$$%\hss
%\binspace0
%\relspace0
\let\quad\relax
\mathalign{
%\Q_1(\XX_1,T)-\Q_1(\XX_1{-}1,T)&=&
%\\&&\hskip-1.5cm{}
%\Q_1(\XX_1{-}1,T)\,(?-(\XX_1{-}1))\, T\hfill\\
\Q_{d}(\XX_d,T)-\Q_{d}(\XX_d{-}1,T)&=&
%\\&&\hskip-1.5cm{}
\Q_{d}(\XX_d{-}1,T)\,(?\,T^{d}-?(\XX_d{-}1)\,T^{d(d_{\Mg}{-}1)})\,,}
$$
dont on déduit, pour tout $i\geq 1$, la majoration
$$
\def\sss#1 {\hbox to1.5em{\hfill(#1)}}
\mathalign{
%\sss i \ddeg\Qdeg{i}_{1}&=&2&+&\ddeg\Qdeg{i{-}1}_{1}\hfill\\
%\sss i 
\ddeg\Qdeg{i}_{d}&\leq &d&+&\sup\Bigset
\ddeg\Qdeg{i-d}_{d},\ 
d+\ddeg\Qdeg{i-d(d_{\Mg}-1)}_{d}/\,,}
\eqnnb\label{Eq-dMg=3-b2=1}$$
où $d(\dMg{-}1)\geq2d$, ce qui permet de prouver par induction sur $i$
$$%\preskip0ex
\mathalign{
\ddeg\Qdeg{i}_{d}(\cg_{d_\Mg}{=}1)&\leq& i\,,&\quad\forall i\geq0\,,\forall d\geq1\,.
}
%\eqnnb\label{Eq-dMg=3-b2=1}
$$
et donc
$$
\displayboxit{
\mathalign{\ddeg\chideg{i}(\cg_{\dMg}{=}1)&\leq& i\,,\quad\forall i\geq0\,,
}}$$

%%%
\item Lorsque $\cg_{\dMg}=0$, la majoration \ref{Eq-dMg=3-b2=1} se simplifie en
$$
\def\sss#1 {\hbox to1.5em{\hfill(#1)}}
\mathalign{
\ddeg\Qdeg{i}_{d}&\leq \sup\Bigset
\ddeg\Qdeg{i-d}_{d},\ 
d+\ddeg\Qdeg{i-d(d_{\Mg}-1)}_{d}/\,,}
%\eqnnb\label{Eq-dMg=3-b2=0}
$$
ce qui permet de prouver par induction sur $i$
$$%\preskip0ex
\mathalign{
\ddeg\Qdeg{i}_{d}(\cg_{\dMg}{=}0)&\leq& 
\smashbot{{i\over\dMg{-}1}}\,,&\quad\forall i\geq0\,,\forall d\geq1\,.
}
%\eqnnb\label{Eq-dMg=3-b2=1}
$$
et donc
$$\preskip0pt
\displayboxit{
\mathalign{\ddeg\chideg{i}(\cg_{\dMg}{=}0)&\leq& 
\smashtop{{i\over\dMg{-}1}}\,,\quad\forall i\geq0\,,
}}$$
ce qui termine la preuve de la proposition.\enddemobox
\end{itemize}
\enddemo


\begin{coro}
Soit\label{theo-stabilite-i-acyclique-betti-BFm} $\Mg$ une pseudovariété $i$-acyclique de type fini de dimension $\dMg\geq1$  et telle que $\dim\Hc^{\dMg}(\Mg;\QQ)\leq1$. 
Alors, pour $i\in\NN$ donné, la famille $\set\Bettibm^{i}(\BFm(\Mg;\QQ))/_{m}$ pour la cohomologie de Borel-Moore est constante pour $m\geq i$. On a aussi,
\begin{enumerate}
%%%
\item si\label{theo-stabilite-i-acyclique-betti-BFm-a} $\dMg=1$, constance sur $\set m\geq 1/$;
%%%
\item si\label{theo-stabilite-i-acyclique-betti-BFm-b} $\dMg=2$ et $\cg_2=0$, nullité sur $\set m>i/$;
%%%
\item si\label{theo-stabilite-i-acyclique-betti-BFm-c} $\dMg\geq3$ et $\cg_{\dMg}=0$, constance sur $\bigset m\geq {i\over\dMg{-}1}/$.
\end{enumerate}
\end{coro}
\demo On applique les estimations de \ref{prop-stabilite-chi-bg} avec $\cg_\dMg\in\set0,1/$. Pour $\dMg=1$, seul le cas $i=0$ et $\cg_0{=}0$ est à considérer. On a pour tout $m\geq1$
$$\mathalign{{1\over m!}\sum_{\alpha\in\Sm}\chideg {0}(\cg_0{=}0,\cg_1)(\alpha)&=&{1\over m!}\sum_{\alpha\in\Sm}(\cg_1)\,\uspp{\XX_1}[-1]\prodnl_{d>1}0\,\uspp{\XX_d}[-d](\alpha)\\\noalign{\kern4pt}
&=&\let\strut\relax\left\{\mathalign{1\text{ si $\cg_1=1$}\\0\text{ si $\cg_1=0$}}\right.\hfill}$$

Les estimations de \ref{prop-stabilite-chi-bg} pour le degré $\ddeg$ des familles de fonctions centrales polynomiales $\chideg i(\cg)$ jointes à la proposition \ref{prop-rang-stabilite-caracteres} justifient les autres assertions à l'exception du cas $\dMg=2$. Dans ce cas, le procédé donne la constance seulement sur $\set m\geq 2i/$. Pour aller plus loin, on remarque que $\chibm\minideg i(\Mg)$ seul dépend des nombre de Betti compacts de $\Mg$. Le cas $\Mg=\CC$ est connu depuis Arnold (\cite{arnold2}) qui montre que la cohomologie rationnelle de $\Bg\Fm(\CC)$ est nulle en degrés $i\geq2$ et est de dimension constante $1$ sur $\set m\geq i/$ pour $i\in\set0,1/$, ce qui règle le cas $i$-acyclique avec $\dMg=2$ et $\cg_1=0$. Le cas $\cg_1>0$ résulte de considérer la suite exacte courte de $\Sm$-modules de \ref{moins-un-point-comparaison}
$$0\to\Hc\big(\Fm ^{\bullet}(\Mg)\big)[-1]\to\Hc(\Fm (\oo\Mg))\to
\Hc(\Fm (\Mg))\to0\eqno(\ast)$$
où $\oo\Mg:=\Mg\mmoins\set \bullet/$ pour un certain $\bullet\in\Mg$, et où $\Fm ^{\bullet}(\Mg)$ est la réunion disjointe des ouverts $\Fm ^{j=\bullet}(\Mg):=\set \cl x\in\Fm  \mid x_i=\bullet/$ où $j=1,\ldots,m$. 
On remarquera ici que $\Hbm^{k}(\Mg)$ et $\Hbm^{k}(\oo\Mg)$ seul diffèrent en degré $d_{\Mg}{-}1$ où 
$$\dim\Hbm^{d_{\Mg}{-}1}(\oo\Mg)=\dim\Hbm^{d_{\Mg}{-}1}(\Mg){+}1\,.$$
En dualisant $(\ast)$ on obtient:
$$0\to
\Hbm^{i}\big(\Fm(\Mg)\big)\to
\Hbm^{i}\big(\Fm(\oo\Mg)\big)\to
\ind_{\Smmo}^{\Sm}\Hbm^{i-(d_{\Mg}{-}1)}\big(\Fmmo(\oo\Mg)\big)\to
0$$
et donc
$$\Betti^{i}(\BFm(\oo\Mg))=\Betti^{i}(\BFm(\Mg))+\Betti^{i-(d_{\Mg}{-}1)}(\BFmm(\oo\Mg))\,.$$

Lorsque $d_{\Mg}=2$, ces remarques montrent que 
$\set\Betti^i(\BFm(\CC\mmoins \cg_1))/_m$ est constante pour $m\geq i$, alors que $\Betti^{1}(\CC\mmoins\cg_1)=\cg_1$. Ceci termine la justification du cas $\dMg=2$, et achève la preuve du corollaire.\enddemo

\subsection{Stabilité de $\set\Bettibm^{i}(\BFm(\Mg))/_{m}$, cas général}\label{stabilite-Betti-cas-general}
On étend la portée du corollaire \ref{theo-stabilite-i-acyclique-betti-BFm} au cas des pseudovariétés générales $\Mg$ orientables. Nous procédons comme dans la preuve du théorème \ref{theo-stabilite-BM-pseudo}, à l'aide de la suite spectrale basique
$$\halfdisplayskips\mathalign{
\IEs(\U^{m})_{1}^{p,q}&=&
\bigoplus_{\hskip-4mm
\tau\in\TTT(\pp,m)
\hskip-4mm}
\ind^{\Sm}_{\HHH_{\utau}\times\S_{m-|\utau|}}
\alt^{d_{\Mg}}\otimes\Hbm^{Q}(\Fg_{\tau}(\Mg_{>0}))\ \Rightarrow\ 
\Hbm^{i}(\Fm(\Mg))}
\postdisplaypenalty10000$$
avec $Q=i-(d_{\Mg}{-}1)(m{-}(\pp))$.

La compatibilité entre les morphismes $p_{m}^{*}:\Hbm^{i}(\Fm(\Mg))\to\Hbm^{i}(\Fmm(\Mg))$ et ceux des suites spectrales basiques (\ref{prop-tableau-normaux-ss-basiques}-(\ref{prop-tableau-normaux-ss-basiques-b}))
$$\IEs(q_m^{*})_{1}^{p,q}:\IEs(\U^{m})^{p,q}_{1}\to\IEs(\U^{\mm})^{\pp,q}_{1}\,,\eqno(\dagger)$$
y compris avec les actions des groupes symétriques, ramènent la question de la stabilité de la famille $\set\Bettibm^{i}(\BFm(\Mg))/_{m}$, à celle de la stabilité des morphismes de suites spectrales de co-invariants (\ref{co-invariants}) induits par $(\dagger)$, \idest
$$\varPhi_{0}(\IEs(q_m^{*})_{1}^{p,q}):
\varPhi_0(\IEs(\U^{m})^{p,q}_{1})\to\varPhi_0(\IEs(\U^{\mm})^{\pp,q}_{1})\,.$$
On est alors emmené à trouver le rang de stabilité des familles de morphismes 
$$
\bigoplus_{\hskip-5mm
\tau\in\TTT(\pp,m)
\hskip-5mm}
\Hbm^{Q}(\Fg_{\tau}(\Mg_{>0}))_{\HHH_{\utau}\times\S_{m-|\utau|}}
\hf{\sum p_{\tau}^{*}}{}{1cm}
\bigoplus_{\hskip-7mm
\tau\in\TTT(p+2,\mm)
\hskip-7mm}
\Hbm^{Q}(\Fg_{\tau}(\Mg_{>0}))_{\HHH_{\utau}\times\S_{\mm-|\utau|}}
\eqno(\diamond)$$
définis par les morphismes de $\HHH_{\utau}$-modules
$$
\varPhi_{\uell}(p_{\tau}^{*}):
\varPhi_{\uell}(\Hbm^{Q}(\Fg_{\tau}(\Mg_{>0}))
\to
\varPhi_{\uell}(\Hbm^{Q}(\Fg_{\tau^{\bullet}}(\Mg_{>0})))
\eqno(\diamond\diamond)$$ 
où $p_{\tau}:\Fg_{\tau^{\bullet}}(\Mg_{>0})\to\Fg_{\tau}(\Mg_{>0})$ est la projection sur les $\pp$ premières coordonnées, et où $\uell$ est tel que $m{-}|\utau|=(\pp){-}\uell$,
conformément à la notation \ref{rema-lambda/m}-(\ref{rema-lambda/m-b}). L'étude de cette question conduit à l'énoncé suivant.

\begin{prop}Soit\label{prop-stabilite-betti-dim3-BFm} $\Mg$ une pseudovariété connexe orientée. Le morphisme 
$$\varPhi_0(p_{m}^{*}):\varPhi_0(\Hbm^{i}(\Fm(\Mg)))\to
\varPhi_0(\Hbm^{i}(\Fmm(\Mg)))$$
 est bijectif pour $m\geq 2i$ si $d_{\Mg}=2$, et pour $m\geq i$ si $d_{\Mg}\geq 3$.
\end{prop}
\demo Soit $\epsilon:=2$ si $d_{\Mg}=2$ et $\epsilon:=1$ si $d_{\Mg}\geq3$.
D'après les remarques préliminaires, la proposition résultera de montrer que les morphismes $\sum p^{*}_{\tau}$ dans $(\diamond)$ sont des isomorphismes pour $m\geq \epsilon i$, ce qui découle clairement de ce que pour tout $m\geq \epsilon i$,
\def\varlistskips{\topsep0cm\itemsep0.5pt\mou\parskip0pt\mou}
\begin{enumerate}
\item le\label{dem-stabilite-betti-dim3-BFm-a} morphisme $\varPhi_{\uell}(p^{*}_{\tau})$
dans $(\diamond\diamond)$ est un isomorphisme;
%%%
\item l'application\label{dem-stabilite-betti-dim3-BFm-b} $(\_)^{\bullet}:\TTT(\pp,m)\to\TTT(p{+2},\mm)$ est bijective pour $Q\geq 0$.
\end{enumerate}

\smallskip
(\ref{dem-stabilite-betti-dim3-BFm-a}) Commençons la généralisation suivante du corollaire \ref{theo-stabilite-i-acyclique-betti-BFm}.

\noindent{\slshape Lemme. Soit $\Xg$ est une pseudovariété $i$-acyclique connexe orientée de dimension $d_{\Xg}\geq2$. Pour tout $t\geq 0$, le morphisme induit
$$\varPhi_{t}(p_{m}^{*}):
\varPhi_{t}(\Hbm^{i}(\Fm(\Xg)))
\to
\varPhi_{t}(\Hbm^{i}(\Fmm(\Xg)))$$
est bijectif pour $m\geq i+t$.}

\begingroup
\parskip0.5ex
\medskip\noindent{\sl Preuve. }On raisonne par induction sur $t\in\NN$ puis, pour chaque $t$ par induction sur $i\in\NN$.
Le cas $t=0$ est réglé pour tout $i\in\NN$, par le corollaire \ref{theo-stabilite-i-acyclique-betti-BFm} modulo le théorème \ref{theo-stabilite-BM-i-acyclique} qui donne le rang de monotonie $m\geq i$. Supposons donc $t>0$ et le lemme vérifié pour $(t{-}1)$.
En dualisant la suite exacte du théorème de scindage \ref{theo-scindage}-(\ref{theo-scindage-a}) et en appliquant le foncteur $\varPhi_{t}(\_)$ (possible puisque $t>0$), on a la suite exacte courte
$$\mathalign{0\to
\bigoplus_{a+b=i}\Hbm^{a}(\Xg)\otimes&
\varPhi_{t-1}(\Hbm^{b}(\Fmmo))\to
\varPhi_{t}(\Hbm^{i}(\Fm))\hfill\\\noalign{\kern-8pt}
&\hskip2mmm{}\to
\varPhi_{t-1}(\ind^{\S_{m-1}}_{\S_{m-2}}\Hbm^{i-(d_{\Xg}-1)}(\Fmmo))
\to
0}
\eqno(\ddagger)$$
qui montre que la bijectivité de $\varPhi_{t}(p_{m}^{*})$  au niveau du terme central est subordonnée par celle des termes extrêmes. 

Lorsque $i=0$, le terme de droite de $(\ddagger)$ est nul puisque $d_{\Xg}>1$ et le lemme résulte des terme de gauche $\varPhi_{t-1}(\Hbm^{b}(\Fg_{m-1}(\Xg)))$ par l'hypothèse inductive.

Lorsque $i>0$, le terme de droite n'est pas forcément nul.
On remarque alors que la preuve du lemme~1~(p.~\pageref{theo-Ind-lambda-Lemme-1}) dans la démonstration du théorème \ref{theo-Ind-lambda}, donnait déjà l'identification
$$\varPhi_{t-1}(\ind^{\S_{m-1}}_{\S_{m-2}}(\_))
\ \simeq\ \
\bigoplusnl_{\cl \alpha\in\big(\biquosb {\S_{m-2} }{\S_{m-1} }{\S_{m-t} }\big)}
(\_)_{\S_{\iii[2,m-1]\cap\alpha \iii[t,m-1]}}\,,
\postskip-0.2ex$$
où 
$$\big|\iii[2,m-1]\cap\alpha \iii[t,m-1]\big|=(m{-}1){-}t'\,,\quad\text{avec $t'\in\iii[t-1,t]$.}$$ On y montrait aussi que l'application naturelle
$$(\_)^{\bullet}_{m}:
\Big(\biquo {\S_{m-2} }{\S_{m-1} }{\S_{m-t} }\Big)
\too
\Big(\biquo {\S_{m-1} }{\S_{m} }{\S_{m-(t-1)} }\Big)
\,,$$
où $\alpha^{\bullet}=\alpha$ sur $\iii[1,m{-}1]$ (donc $\alpha^{\bullet}(m)=m$), est bijective dès que
$m\geq t+1\,.$

De ces remarques, suit que sur les termes de droite de $(\ddagger)$, l'application
$$
\varPhi_{t-1}(\ind^{\S_{m-1}}_{\S_{m-2}}(\Hbm^{i-(d_{\Xg}-1)}(\Fmmo)))\to
\varPhi_{t-1}(\ind^{\S_{m}}_{\S_{m-1}}(\Hbm^{i-(d_{\Xg}-1)}(\Fm)))\eqno(\ast)$$
sera bijective dès lors que 
$$m\geq i+t\,.\eqno(\diamond)$$
En effet, pour que $(\ast)$ soit bijective, il suffit de vérifier que
\def\varlistskips{\itemsep0pt\mou\parsep0pt\parskip0pt\topsep2pt
\def\theenumi{\roman{enumi}}
\def\labelenumi{{\rm\theenumi)}}}
\begin{enumerate}
\item l'application\label{prop-stabilite-betti-dim3-BFm-lemme-a} $(\_)^{\bullet}_{m}$ est bijective, donc que $m\geq t+1$;

\item l'application\label{prop-stabilite-betti-dim3-BFm-lemme-b} $\varPhi_{t'}(\Hbm^{i-(d_{\Xg}-1)}(\Fmmo))\to
\varPhi_{t'}(\Hbm^{i-(d_{\Xg}-1)}(\Fm))$ est bijective pour $t'\in\iii[t-1,t]$, donc, que $m{-}1\geq i{-}(d_{\Xg}{-}1){+}t'$, par hypothèses inductives puisque $i{-}(d_{\Xg}{-}1)<i$ et $t'\leq t$;
\end{enumerate}
et comme $i\geq 1$, la condition $(\diamond)$ suffit pour avoir 
(\ref{prop-stabilite-betti-dim3-BFm-lemme-a},\ref{prop-stabilite-betti-dim3-BFm-lemme-b}), ce qui termine la preuve du lemme.
 \hfill$\boxminus$
\endgroup

\smallskip
Revenons à  la preuve de l'assertion (\ref{dem-stabilite-betti-dim3-BFm-a}). Lorsque $d_{\Mg}\geq 1$, le lemme s'applique aux morphismes $(\diamond\diamond)$
$$
\varPhi_{\uell}(p_{\tau}^{*}):
\varPhi_{\uell}(\Hbm^{Q}(\Fg_{\tau}(\Mg_{>0})))
\to
\varPhi_{\uell}(\Hbm^{Q}(\Fg_{\tau^{\bullet}}(\Mg_{>0})))
$$ 
et montre que
$\varPhi_{\uell}(p_{\tau}^{*})$ est bijective sous les conditions
$$\bigpar (p{+}1)\geq (Q{+}\uell)
/\text{\quad ou bien\quad }\bigpar Q< 0/
\,.\eqno(\ddagger)$$
%où $\uell$ désigne le nombre des lignes du tableau $\utau$ (\cf  \ref{rema-lambda/m}-(\ref{rema-lambda/m-b})).

En substituant (\cf notations  \ref{rema-lambda/m}-(\ref{rema-lambda/m-b}))
$$\binspace1\pmathalign{
Q&\leftrightarrow&i-(d_{\Mg}-1)(m-(\pp))\,,\\
\uell&\leftrightarrow&|\utau|-(m-(\pp))\,,\hfill\\
m{-}(\pp)&\leftrightarrow&|\utau|-\uell\,,\hfill}$$ 
la première condition dans $(\ddagger)$ s'écrit aussi
$$%\binspace1
\bigpar m\geq i-(d_{\Mg}{-}2)|\utau| + (d_{\Mg}{-}1)\uell/
\,,\eqno(\ddagger\ddagger)$$
et comme $|\utau|\geq2\uell$, on voit aisément que si $d_{\Mg}=2$, l'intervalle $\set m\geq 2i/$ est conforme à  $(\ddagger\ddagger)$, tandis que si $d_{\Mg}\geq3$, c'est le cas de $\set m\geq i/$.

\smallskip
(\ref{dem-stabilite-betti-dim3-BFm-b}) On raisonne par l'absurde. 
Nous avons vu dans la preuve du théorème \ref{theo-stabilite-BM-pseudo}-(\ref{theo-rang-pseudovariete-b}) (p.~\pageref{bullet-non-bijective}) que l'application $(\_)^{\bullet}$ n'est pas bijective si et seulement si, $2(\pp)<m$. Dans ce cas, si $m\geq\epsilon i$, on a
$$\preskip1exQ=i{-}(m{-}(\pp))
<i-(d_\Mg{-}1){m\over 2}\leq 
\bigpar{(2/\epsilon){+}1{-}d_{\Mg}}/{m\over 2}\leq 0\,,$$
puisque $d_{\Mg}\geq 2$, ce qui est contraire à la condition $Q\geq 0$.\enddemo
%
%\begin{prop}Si\label{prop-stabilite-betti-dim<3-BFm} \color{red}$\Mg$ est une variété connexe orientée de dimension $\dMg=2$, le morphisme 
%$$\varPhi_0(p_{m}^{*}):\varPhi_0(\Hbm^{i}(\Fm(\Mg)))\to
%\varPhi_0(\Hbm^{i}(\Fmm(\Mg)))$$
% est bijectif pour $m> i$.
%\end{prop}
%\demo
%\enddemo



























